Advancing Beyond Identification: Multi-bit Watermark for Large Language Models

We show the viability of tackling misuses of large language models beyond the identification of machine-generated text. While existing zero-bit watermark methods focus on detection only, some malicious misuses demand tracing the adversary user for counteracting them. To address this, we propose Multi-bit Watermark via Position Allocation, embedding traceable multi-bit information during language model generation. Through allocating tokens onto different parts of the messages, we embed longer messages in high corruption settings without added latency. By independently embedding sub-units of messages, the proposed method outperforms the existing works in terms of robustness and latency. Leveraging the benefits of zero-bit watermarking, our method enables robust extraction of the watermark without any model access, embedding and extraction of long messages ($\geq$ 32-bit) without finetuning, and maintaining text quality, while allowing zero-bit detection all at the same time. Code is released here: https://github.com/bangawayoo/mb-lm-watermarking

==> sections/0031-method.tex <==


% Method 


The objective of multi-bit watermarking is to embed and extract a message $\mathbf{m} \in \Sigma^b$ where $\Sigma$ denotes the $r$-nary possible strings, or more commonly referred to as the alphabet. For a binary message, $\Sigma=\{0,1\}$.  We let $p \in \{0, \dots, b-1\}$ denote the position of the message and $\mathbf{m}[p] \in \{0, \dots, r-1\}$ the message content at that position. Hereafter, we use $[a]$ to denote the integer set $\{0, \dots, a-1\}$. Our proposed method \textbf{M}ulti-bit watermarking via \textbf{P}osition \textbf{A}llo\textbf{c}ation (MPAC) works by allocating the tokens to message positions.




\subsection{Zero-bit Watermarking \citep{kirchenbauer2023watermark}}\label{subsec:zwb}
A watermark is embedded by biasing the language model to output a certain subset of tokens. 
Given an autoregressive language model that predicts the next token with vocabulary $V$,
a subset of tokens is randomly selected from the vocabulary at each token step $t$ and forms a green list $\mathcal{G}_t$. The logit scores  $l_t \in \mathbb{R}^{|V|}$ are modified towards selecting the green-listed tokens in favor of the other tokens by adding a bias term $\delta$ to the logits in $\mathcal{G}_t$. Instead of fixing the greenlist using rule-based heuristics such as spelling or synonym variations \citep{he2022protecting}, the greenlist is selected (pseudo-)randomly at each time step to minimize a noticeable shift in text distributions. At each time step, a seed $s$ is outputted depending on the previous $h$ tokens using a pseudo-random function $f: \mathbb{N}^h \rightarrow \mathbb{N}$, and $s$ is used to sample $\mathcal{G}_t$ from $V$. 

At decoding, the greenlist can be recovered by using the same pesudo-random function $f$. The presence of a watermark is determined by counting the number of tokens in the greenlist. For a human-generated text that has no knowledge of the greenlist rule, a token will be from the greenlist with the probability $\gamma \leq 0.5$, the proportion of the greenlist size compared to the entire vocabulary. Without the knowledge of the greenlist (null hypothesis), the number of tokens in the greenlist ($g$) follows a binomial distribution. \citep{kirchenbauer2023watermark} used the normal approximation to the binomial distribution to compute the $z$-statistics for a text with $T$ tokens: $z = \frac{g - \gamma T}{\sqrt{\gamma(1-\gamma)T}}$. 


\subsection{MPAC: Extending to Multi-bit Watermark}
\label{subsec:multibit}
 First, notice that zero-bit watermarking can be viewed as watermarking a single bit of information stating the existence of a watermark ($\mathbf{m}$=0). In essence, each token generated by the language model is a signal in favor of the watermark (See Fig.~\ref{fig:multi-bit}-Right). 

An autoregressive language model $p(\cdot|x)$ predicts the probability distribution over the next token $\Delta(V)$ given arbitrary length prefix tokens. For the $t^{\text th}$ token, the message encoding function $\mathcal{E}:\Sigma^{b} \times \Delta(V) \rightarrow \Delta(V)$ generates another distribution dependent on the message. In our MPAC, we first assign a position $p$  using a random number generator seeded with $s$. Then the message content $m=\mathbf{m}[p]$ is encoded by permuting $V$ and favoring the $m^{\text{th}}$ subset. Our method is extremely easy to implement over the zero-bit watermarking scheme. We highlight the steps in colors that are specific to ours. Given $t-1$ prefix tokens $X_{1:t-1}$, bit message $\mathbf{m}$, and pseudo-random function $f$, the $t^\text{th}$ token is generated by 


\begin{enumerate}[noitemsep]
    \item Compute hash of tokens $s=f(X_{t-h:t-1})$. Use $s$ as a seed for a random number generator.
    \item \hlc[cyan!40]{$p \leftarrow \texttt{sample}([b])$} \textcolor{blue}{\qquad \# $p$ is the position of the message.}
    \item \hlc[cyan!40]{$m \leftarrow \mathbf{m}[p]$} \textcolor{blue}{\qquad\qquad \ \ \# $m$ is the message content at position $p$.}
    \item Permute vocabulary $\mathcal{V}_t$ using $s$ as seed.
    \item \hlc[cyan!40]{Partition $\mathcal{V}_t=[\mathcal{C}_t^{0}, \cdots , \mathcal{C}_t^{r-1}]$ discarding remainders if any.}
    \item Add $\delta$ to token logits in $\mathcal{C}_t^{m}$.
\end{enumerate}

\noindent where $r$ is the number of available partitions. The number of vocabulary partitions is determined by the greenlist proportion $\gamma$, i.e. $r = \lfloor \frac{1}{\gamma} \rfloor$.  When $r>2$, we can further increase the load capacity by taking advantage of all the 'colored' lists, instead of only using the greenlist. Given a binary message of length $b$, the message is convereted to radix $r$ attaining $\mathbf{m}_r \in [r]^{\tilde b}$ where $\tilde b=\lceil \frac{b}{\log_2{r}} \rceil $.  In Figure \ref{fig:multi-bit} Left, we illustrate the case of $r=4$ and $b=8$, where the 8-bit message is converted into radix $4$, resulting in an effective message length of 4 ($\tilde b=4$)\footnote{Hereafter, we use $b$ instead of $\tilde b$ to denote the effective message length (dimension of $\mathbf{m}_r$).}. At each token generation, the message content at the assigned position $p$ determines which colorlist to add $\delta$ to. If the message content is `0', the tokens from the first list (red in Fig. \ref{fig:multi-bit}) are favored. Note that zero-bit watermarking can be seen as a special case of embedding the same single bit message ($b=1, \mathbf{m}=0$) as shown in Figure \ref{fig:multi-bit}-Right.  


\begin{figure*}[t]
    \vspace{-3mm}
    \centering
    \includegraphics[width=\textwidth]{fig/overview.png}
    \caption{An overview of our method MPAC. The number inside a token (e.g. $\boxed{p=1}$) denotes the allocated position, while the color signifies the message content at that position. At Step 1, a position is sampled prior to generating a token. At Step 2, the message at that position determines the token subsets to favor. \textit{Right:} Zero-bit watermarking can be viewed as a special case of multi-bit watermarking.} 
    \label{fig:multi-bit}
\vspace{-4mm}
\end{figure*}

\noindent \textbf{Message Decoding}
Given a watermarked language model output, we determine the position and which colorlist each token is from and increment the number of tokens in the colored lists. For instance, for the $t^\text{th}$ token with message position $p=i$ and the $j^{\text{th}}$ colorlist $\mathcal{C}_t^j$, we increment the counter $\mathbf{W}_i[j]$. After computing this on the entire text segment, we predict the message content by taking the colorlist with the most tokens for each position. A more detailed algorithm is shown in \edit{Algorithm \ref{alg:extraction}}. 


\SetKwInput{KwInput}{Input}              
\SetKwInput{KwOutput}{Output}  
\maketitle
    \begin{algorithm*}[t]
    \DontPrintSemicolon
    \SetNoFillComment
        \KwInput{Watermarked text $X_{1:T}$, hash context width $h$, effective message length $\tilde b$}
        \KwOutput{Predicted message $\hat{\textbf{m}}$, number of colorlisted tokens $w$}
        \begin{multicols}{2}
        \tcc{Initialize counter}
        {$\textbf{W}_{p}[m] = 0 \text{   } \forall p,m$}\; 
        \tcc{Count tokens in colorlists}
        \For{$t \texttt{ in } [h+1, T]$}
        {
            $s=f(X_{t-h:t-1})$\;
            $p=\texttt{sample}([\tilde b])$ \;
            \For{$m \texttt{ in }[r]$}
            {
                Permute $\mathcal{V}_t$ using $s$ as seed\;
                \If{$X_t \in \mathcal{G}_t^{m}$}
                    {
                    $\textbf{W}_{p}[m]$ += 1 \;
                    }
            }
            
        }
        \tcc{Predict message}
        $\hat{\textbf{m}}_r = \text{`` "}$\; 
        $w=0$\;
        \For{$p \texttt{ in } [\tilde b]$}
        {
            $w$ += $\texttt{max}(\textbf{W}_{p}[m])$\;
            $\hat{m}=\texttt{argmax}_m(\mathbf{W}_p[m])$\;
            $\hat{\textbf{m}}_r$ += $\texttt{str}(\hat{m}$) \; 
        }
        Get bit message $\hat{\textbf{m}}$ by converting $\hat{\textbf{m}}_r$ \;
        \Return $\hat{\textbf{m}}$, $w$
    \end{multicols}
\caption{Message Decoding}
\label{alg:extraction}
\end{algorithm*}

\subsubsection{Comparison to Other Works}
The message encoding function of \citet{fernandez2023three} and \citet{wang2023towards} both use the entire message $\mathbf{m}$. For \citet{fernandez2023three}, once permuting the vocabulary list as done in ours, they cyclically shift the vocabulary $m_{10}$ time where $m_{10}$ is the radix-10 form of $\textbf{m}$. This provides the same signal every token that is unique to each message. Similarly, \citet{wang2023towards} hashes $\textbf{m}$ to attain a seed $s'$ to permute the vocabulary along with the seed attained from prefix tokens. 

Using the entire message leads to two key characteristics that diverge from ours. First, the hamming distance between two messages is not translated after applying the encoding function. As an example, consider the message encoding function of \citealt{wang2023towards}. Seeding the random number generator from the hash value of $\textbf{m}=0000$  is not any closer to $\textbf{m}=0001$ (hamming distance of 1) as it is to $\textbf{m}=1111$ (hamming distance of 4). This leads to an all-or-nothing behavior where either the entire message is extracted without error or is a completely random message. In the presence of high corruption, which reflects the real-world case, we show this behavior is not desireable as it lacks enough signal to correctly predict the message.

In addition,  the exponential number of messages ($\bigO(2^b)$)  should be considered during message decoding to find the optimal message, which renders embedding long messages ($\geq 32$-bit) extremely computation-heavy\footnote{See Section 7.5 of \citealp{wang2023towards}
} . For \citealt{fernandez2023three}, the message encoding phase is also affected by the bit-width due to the cyclic shift operation, which is more problematic as it affects the end users. MPAC encodes and decodes each bit position of the message independently, which brings a negligible increase in the computation as the message length is increased.

The simplicity of our multi-bit watermark scheme via position allocation makes it generalizable to applying it on top of other methods. Using the position allocation scheme, we decompose the multi-bit message into blocks and hierarchically embed them using the message encoding scheme of \citet{fernandez2023three}. We dub this as Block Allocation and show in the subsequent section that this enables the prior work to embed longer messages. An example of generalizing to other zero-bit watermark approach is  provided in Appendix \ref{appendix:other-zwb}.



\subsection{Detecting Machine Text}\label{subsec:detection}
\begin{comment}
While we can use MPAC to decode the multi-bit watermark in conjunction with another detection mechanism, MPAC alone can detect human text from watermarked text just like zero-bit watermarking.The strength of our watermark can be determined by taking the maximum cell frequency of each position, which is modeled by the confidence $c_i$ at each position. 
\end{comment}
To distinguish between a watermarked text and a non-watermarked (human-written) text, we count the number of tokens assinged to the predicted message. This corresponds to $C$  in Line 12 of Algo. alg:extraction. We model the number of tokens in the argmax colorlist of position $i$ as a random variable $C_i \distas{H_0} \text{Binomial}(T_i, \gamma$) where $T_i$ is the number of tokens assigned to position $i$. 
As $C_0, \dots, C_{b-1}$ are independent for a fixed set of trials ($T_i, \dots, T_{b-1}$) and have the same success probability parameter, the sum of these is a binomial random variable as well:
\begin{equation}\label{eq:zero-bit-detection}
    C = C_0 + \cdots + C_{b-1} \distas{H_0} \text{Binomial}(T, \gamma)
\end{equation}
where $T=T_{0}+\cdots+T_{b-1}$. This reduces to the same random variable used in zero-bit watermarking and we can compute the z-statistics from \cref{subsec:zwb}. More discussion regarding other possible statistics is outlined in the last section of Appendix \ref{appendix:detection-analysis}. 

